Consistency of empirical distributions of sequences of graph statistics in networks with dependent edges

One of the first steps in applications of statistical network analysis is frequently to produce summary charts of important features of the network. Many of these features take the form of sequences of graph statistics counting the number of realized events in the network, examples of which include the degree distribution, as well as the edgewise shared partner distribution, and more. We provide conditions under which the empirical distributions of sequences of graph statistics are consistent in the $\ell_{\infty}$-norm in settings where edges in the network are dependent. We accomplish this by elaborating a weak dependence condition which ensures that we can obtain exponential inequalities which bound probabilities of deviations of graph statistics from the expected value. We apply this concentration inequality to empirical distributions of sequences of graph statistics and derive non-asymptotic bounds on the $\ell_{\infty}$-error which hold with high probability. Our non-asymptotic results are then extended to demonstrate uniform convergence almost surely in selected examples. We illustrate theoretical results through examples, simulation studies, and an application.

==> preamble.tex <==
%% Package declarations 
\usepackage[mathscr]{eucal}
\usepackage{centernot}
\usepackage{hyperref}
\usepackage{dlfltxbcodetips}
%\usepackage{bbm}
%\usepackage{mathtools}
\usepackage{subfigure}
%\usepackage{amsfonts}
%%\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{fancybox}
\usepackage{graphicx}
\usepackage{bm}
%\usepackage{latexsym}
\usepackage[dvipsnames]{xcolor}

%% Library declarations 

\RequirePackage[draft]{fixme}


\definecolor{myyellow}{RGB}{250, 218, 94}
\definecolor{myred}{RGB}{255, 75, 70}
\definecolor{myblue}{RGB}{0, 135, 189}
\definecolor{mypink}{RGB}{252, 137, 172}
\definecolor{mygrey}{RGB}{211,211,211} 
\definecolor{myorange}{RGB}{255, 159, 0}

%% Symbol commands 

\newcommand{\change}{\color{Maroon}}

\newcommand{\jstew}{\bf \color{WildStrawberry}}
\newcommand{\jli}{\color{orange}}

\newcommand{\dpath}{\centernot{\longleftrightarrow}}


% hats, stars, & dots
\newcommand{\Mle}{\widehat\bTheta}
\newcommand{\mle}{\widehat\btheta}
\newcommand{\mple}{\widetilde\btheta}
\newcommand{\Mple}{\widetilde\bTheta}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\certf}{\text{cert}(f)}
\newcommand{\zstar}{\bz^\star}
\newcommand{\Thetastar}{\Theta^\star}
\newcommand{\thetastar}{\theta^\star}
\newcommand{\etastar}{\eta^\star}
\newcommand{\thetadot}{\dot\theta}
\newcommand{\bthetadot}{\dot\btheta}
\newcommand{\zhat}{\widehat{\bz}}
\newcommand{\zdot}{\dot\bz}
\newcommand{\thetahat}{\widehat{\theta}}
\newcommand{\Var}{\mathop{Var}}
\newcommand{\Cov}{\mathop{Cov}} 
\newcommand{\vech}{\mbox{vech}}
\newcommand{\pl}{\widetilde\ell}
\newcommand{\plkij}{\widetilde\ell_{k,k,\{i,j\}}}
\newcommand{\plklij}{\widetilde\ell_{k,l,\{i,j\}}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\dep}{\bm{\mcD}_N}
\newcommand{\bfun}{\widetilde{b}_{k,i}(\bx)}
\newcommand{\mdelta}{\delta_{i,j,k}}
\newcommand{\muk}{\mu_k}

\newcommand{\emp}{\widehat{F}_N(\bX)}
\newcommand{\empnox}{\widehat{F}_N}
\newcommand{\empk}{\widehat{F}_{N,k}(\bX)}
\newcommand{\empd}{\widehat{F}_{N,d}(\bX)}
\newcommand{\empo}{\widehat{F}_{N,0}(\bX)}
\newcommand{\empp}{\widehat{F}_{N,p}(\bX)}

\newcommand{\edges}{|\mE|}
\newcommand{\truth}{F_N}
\newcommand{\truthk}{F_{N,k}}

% Text in math
\newcommand{\rint}{\mathop{\mbox{rint}}}
\newcommand{\mdim}{\mbox{dim}}
\newcommand{\interior}{\textnormal{int}}
\newcommand{\cert}{\textnormal{cert}}
\newcommand{\su}{\sup\limits}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\tv}{{\tiny\mbox{TV}}}
\newcommand{\lip}{{\tiny\mbox{Lip}}}
\newcommand{\rank}{\textnormal{rank}}
\newcommand{\dimd}{m}
\newcommand{\defined}{\overset{\scalebox{0.75}{def}}{=}}


% \mathscr
\newcommand{\mA}{\mathscr{A}}
\newcommand{\mB}{\mathscr{B}}
\newcommand{\mC}{\mathscr{C}}
\newcommand{\mD}{\mathscr{D}}
\newcommand{\mE}{\mathscr{E}}
\newcommand{\mF}{\mathscr{F}}
\newcommand{\mG}{\mathscr{G}}
\newcommand{\mmG}{\mathfrak{N}}
\newcommand{\mH}{\mathscr{H}}
\newcommand{\mJ}{\mathscr{J}}
\newcommand{\mK}{\mathscr{K}}
\newcommand{\mL}{\mathscr{L}}
\newcommand{\mM}{\mathscr{M}}
\newcommand{\mN}{\mathscr{N}}
\newcommand{\mO}{\mathscr{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mQ}{\mathscr{Q}}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\mS}{\mathscr{S}}
\newcommand{\mT}{\mathscr{T}}
\newcommand{\mU}{\mathscr{U}}
\newcommand{\mV}{\mathscr{V}}
\newcommand{\mW}{\mathscr{W}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathscr{Y}}
\newcommand{\mZ}{\mathscr{Z}}


% \mathcal
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcI}{I}
%\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcJ}{\mathcal{J}}
\newcommand{\mcK}{\mathcal{K}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcS}{\mathbb{S}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcZ}{\mathcal{Z}}




%  \mathbb
\newcommand{\mbA}{\mathbb{A}}
\newcommand{\mbB}{\mathbb{B}}
\newcommand{\mbC}{\mathbb{C}}
\newcommand{\mbD}{\mathbb{D}}
\newcommand{\mbE}{\mathbb{E}}
\newcommand{\mbF}{\mathbb{F}}
\newcommand{\mbG}{\mathbb{G}}
\newcommand{\mbH}{\mathbb{H}}
\newcommand{\mbI}{\mathbb{I}}
\newcommand{\mbJ}{\mathbb{J}}
\newcommand{\mbK}{\mathbb{K}}
\newcommand{\mbL}{\mathbb{L}}
\newcommand{\mbM}{\mathbb{M}}
\newcommand{\mbN}{\mathbb{N}}
\newcommand{\mbO}{\mathbb{O}}
\newcommand{\mbP}{\mathbb{P}}
\newcommand{\mbQ}{\mathbb{Q}}
\newcommand{\mbR}{\mathbb{R}}
\newcommand{\mbS}{\mathbb{S}}
\newcommand{\mbT}{\mathbb{T}}
\newcommand{\mbU}{\mathbb{U}}
\newcommand{\mbV}{\mathbb{V}}
\newcommand{\mbW}{\mathbb{W}}
\newcommand{\mbX}{\mathbb{X}}
\newcommand{\mbY}{\mathbb{Y}}
\newcommand{\mbZ}{\mathbb{Z}}


% \bm -- lowercase
\newcommand{\bma}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bmi}{\bm{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\mathscr{P}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}

% \bm -- uppercase 
\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}

% bold greek
\newcommand{\balpha}{\bm\alpha}
\newcommand{\bphi}{\mbox{\boldmath$\phi$}}
\newcommand{\bbeta}{\mbox{\boldmath$\beta$}}
\newcommand{\bgamma}{\mbox{\boldmath$\gamma$}}
\newcommand{\blambda}{\mbox{\boldmath$\lambda$}}
\newcommand{\brho}{\mbox{\boldmath$\rho$}}
\newcommand{\bmu}{\mbox{\boldmath$\mu$}}
\newcommand{\bomega}{\mbox{\boldmath$\omega$}}
\newcommand{\bsigma}{\mbox{\boldmath$\sigma$}}
\newcommand{\bSigma}{\mbox{\boldmath$\Sigma$}}
\newcommand{\bTheta}{\bm\Theta}
\newcommand{\bta}{\boldsymbol{\eta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\hatbtheta}{\boldsymbol{\hat{\theta}}}
\newcommand{\bvartheta}{\mbox{\boldmath$\vartheta$}}
\newcommand{\bpi}{\mbox{\boldmath$\pi$}}
\newcommand{\bxi}{\mbox{\boldmath$\xi$}}
\newcommand{\bXi}{\mbox{\boldmath$\Xi$}}
\newcommand{\bPsi}{\mbox{\boldmath$\Psi$}}
\newcommand{\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand{\bLambda}{\mbox{\boldmath$\Lambda$}}
\newcommand{\bPhi}{\mbox{\boldmath$\Phi$}}
\newcommand{\bnu}{\mbox{\boldmath$\vartheta$}}
\newcommand{\bupsilon}{\mbox{\boldmath$\upsilon$}}
\newcommand{\bUpsilon}{\mbox{\boldmath$\Upsilon$}}



% General Math Symbols 
\newcommand{\msim}{\mathop{\rm \sim}}
\newcommand{\one}{\mathbbm{1}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\newcommand\orth{\protect\mathpalette{\protect\independenT}{\perp}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\tends}{\longrightarrow}
\newcommand{\tend}{\rightarrow}
\newcommand{\define}{\mathop{=}\limits^{\mbox{\tiny def}}}
\newcommand{\law}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize d}}}
\newcommand{\as}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize a.s.}}}
\newcommand{\ind}{\msim\limits^{\mbox{\tiny ind}}}
\newcommand{\iid}{\msim\limits^{\mbox{\tiny iid}}}
\renewcommand{\bar}{\overline}
\newcommand{\dsum}{\displaystyle\sum\limits}
\newcommand{\dint}{\displaystyle\int\limits}
\newcommand{\dprod}{\displaystyle\prod\limits}
\newcommand{\dd}{\mathop{\mbox{d}}\nolimits}
\newcommand{\gradient}{\mathop{\nabla}\nolimits}
\DeclareMathOperator*{\ri}{\mbox{ri}}
\DeclareMathOperator*{\cl}{\mbox{cl}}
\newcommand{\var}{\mathbb{V}}
\newcommand{\cov}{\mathbb{C}}
\newcommand{\norm}[1]{||#1||} 
\newcommand{\mnorm}[1]{|||#1|||}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\natspace}{\bm{\mathfrak{N}}}
\newcommand{\mmax}{{\tiny \mbox{max}}}
\newcommand{\sepmodel}{\mbP_{\nat}}
\newcommand{\sepfam}{\mcF}
\newcommand{\gradW}{\gamma_{W}(\nat_W, \bx)}
\newcommand{\GradW}{\gamma_{W}(\nat_W, \bX)}
\newcommand{\gradB}{\gamma_{B}(\nat_B, \bx)}
\newcommand{\GradB}{\gamma_{B}(\nat_B, \bX)}
\newcommand{\gradLW}{\gamma_{k,k}(\nat_W, \bx_{\mA_k})}
\newcommand{\gradLB}{\gamma_{k,l}(\nat_B, \bx_{\mA_k,\mA_l})}
\newcommand{\GradLW}{\gamma_{k,k}(\nat_W, \bX_{\mA_k})}
\newcommand{\GradLB}{\gamma_{k,l}(\nat_B, \bX_{\mA_k,\mA_l})}
\newcommand{\Lam}{\xi_{\epsilon^\star} \; \mbE \, \norm{\bY}_1}
\newcommand{\LamPL}{\widetilde\xi_{\epsilon^\star} \; \mbE \, \norm{\bY}_1}
\newcommand{\gradPL}{\widetilde\gamma_{\nat}(\bx)}
\newcommand{\GradPL}{\widetilde\gamma_{\nat}(\bX)}
\newcommand{\phiN}{\phi_N(\truth)}
\newcommand{\mbXkij}{\mbX_{k,k,\{i,j\}}^{\bx}} 
\newcommand{\mbXklij}{\mbX_{k,l,\{i,j\}}^{\bx}}
\newcommand{\mbEkij}{\mbE_{\{i,j\},\btheta_W}^{\bx}}
\newcommand{\mbEklij}{\mbE_{\{i,j\}, \btheta_B}^{\bx}}
\newcommand{\mlewprob}{\ldots}
\newcommand{\mlebprob}{\ldots}
\newcommand{\tbR}{\widetilde\bR}
\newcommand{\tbD}{\widetilde\bD}
\newcommand{\natw}{\nat_W}
\newcommand{\natb}{\nat_B}


% begin/end enviornment commands
\newcommand{\btt}{\begin{box}}
\newcommand{\ett}{\end{box}}

\newcommand{\btheorem}{\begin{bclogo}[couleur={rgb:orange,0;yellow,0;white,1},arrondi=0.1,logo=\bcplume,ombre=true]{Theorem}}
\newcommand{\ettheorem}{\end{bclogo}}

\newcommand{\bst}{\begin{bclogo}[couleur={rgb:orange,1;yellow,1;white,0.5},arrondi=0.1,logo=\bcpanchant]}
\newcommand{\est}{\end{bclogo}}

\newcommand{\ba}{\begin{array}{llllllllll}}
\newcommand{\ea}{\end{array}}

\newcommand{\bea}{\begin{equation}\begin{array}{llllllllll}}
\newcommand{\eea}{\end{array}\end{equation}}

\newcommand{\be}{\begin{equation}\begin{array}{lllllllllllllllll}}
\newcommand{\beno}{\begin{equation}\begin{array}{lllllllllllll}\nonumber}
\newcommand{\ee}{\end{array}\end{equation}}

\newcommand{\bel}{\begin{equation}\begin{array}{lllllllllllll}\nonumber}
\newcommand{\eel}{\Box\end{array}\end{equation}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}

\newcommand{\bbq}{\begin{quote}\bf\em}
\newcommand{\ebq}{\end{quote}}



% Proof language / math env symbol commands -- to be used in \be \ee enviornments 
\newcommand{\wrt}{&\mbox{wrt}&}
\renewcommand{\forall}{&\mbox{for all}&}
\newcommand{\andd}{&\mbox{and}&}
\renewcommand{\=}{&=&}
\newcommand{\less}{&<&}
\newcommand{\lte}{&\leq&}
\newcommand{\gte}{&\geq&}
\newcommand{\ase}{& \mathop{\widehat{=}} &}





% Latex editor helpers
\newcommand{\dis}{\displaystyle}
\newcommand{\hide}[1]{}
\newcommand{\ghost}[1]{}
\newcommand{\alert}{\textcolor{red}}
\newcommand{\s}{\vspace{0.25cm}}
\newcommand{\ls}{\vspace{.15cm}}
\newcommand{\hs}{\hspace{0.25cm}}
\newcommand{\lef}{\left(}
\newcommand{\rig}{\right)}
\newcommand{\cont}{\alert{Please continue here...}}
\newcommand{\fs}{\footnotesize}
\newcommand{\ti}{\tiny}




% Theorem, Proof, Remark, etc. enviornments
%\newcounter{comment}
%\newenvironment{comment}[1][]{\refstepcounter{comment}\par\smallskip\noindent%
%\textbf{Comment~\thecomment #1}:\vspace{0.25cm}\\ \rmfamily}{}
%\newcommand{\bcom}{\begin{comment}\em}
%\newcommand{\ecom}{\end{comment}}

\newcounter{ex}
\newenvironment{ex}[1][]{\refstepcounter{ex}\par\smallskip\indent%
\textbf{Example~\theex #1.} \rmfamily}{}

\newcounter{counterexample}
\newenvironment{counterexample}[1][]{\refstepcounter{counterexample}\par\medskip\indent%
\textbf{Counterexample~\thecounterexample #1}: \rmfamily}{\medskip}





\newcounter{ttproof}
\setcounter{ttproof}{0}
\newcommand{\ttproof}{%
\addtocounter{ttproof}{1}%
{\medskip}\textsc{Proof of Theorem}{}
}

\newcounter{pproof}
\setcounter{pproof}{0}
\newcommand{\pproof}{%
\addtocounter{pproof}{1}%
{\medskip}\textsc{Proof of Proposition}{}
}


\newcounter{ccproof}
\setcounter{ccproof}{0}
\newcommand{\ccproof}{%
\addtocounter{ccproof}{1}%
{\medskip}\textsc{Proof of Corollary}{}
}

\newcounter{ccsproof}
\setcounter{ccsproof}{0}
\newcommand{\ccsproof}{%
\addtocounter{ccsproof}{1}%
{\medskip}\textsc{Proof of Corollaries}{}
}


\newcounter{llproof}
\setcounter{llproof}{0}
\newcommand{\llproof}{%
\addtocounter{llproof}{1}%
{}\textsc{Proof of Lemma}{}
}



\newcounter{com}
\newenvironment{com}[1][]{\refstepcounter{com}\par\medskip\indent%
\textit{Remark~\thecom #1}. \rmfamily}{\medskip}

\newcounter{assumption}
\newenvironment{assumption}[1][]{\refstepcounter{assumption}\par\noindent%
\textbf{Assumption~A.\theassumption #1}. \rmfamily}{\medskip}

\def\define{\mathop{=}\limits^{\mbox{\tiny def}}}

\newcommand{\nei}{\mbox{ne}} 


\newcommand{\Smaller}[1][]{\mbox{\scriptsize$#1$}}

\newcommand{\vol}{\mbox{Vol}}

\newcommand{\nat}{\btheta}
\newcommand{\Nat}{\bTheta}

\DeclareMathOperator{\trace}{trace}


\newcommand{\ip}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize p}}}
\newcommand{\ipshort}{\mathop{\rightarrow}\limits^{\mbox{\footnotesize p}}}


==> short_preamble.tex <==

%% Symbol commands 

\newcommand{\change}{\color{red}}


% hats, stars, & dots
\newcommand{\Mle}{\widehat\bTheta}
\newcommand{\mle}{\widehat\btheta}
\newcommand{\mple}{\widetilde\btheta}
\newcommand{\Mple}{\widetilde\bTheta}
\newcommand{\truth}{\btheta^\star}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\certf}{\text{cert}(f)}
\newcommand{\zstar}{\bz^\star}
\newcommand{\Thetastar}{\Theta^\star}
\newcommand{\thetastar}{\theta^\star}
\newcommand{\etastar}{\eta^\star}
\newcommand{\thetadot}{\dot\theta}
\newcommand{\bthetadot}{\dot\btheta}
\newcommand{\zhat}{\widehat{\bz}}
\newcommand{\zdot}{\dot\bz}
\newcommand{\thetahat}{\widehat{\theta}}
\newcommand{\Var}{\mathop{Var}}
\newcommand{\Cov}{\mathop{Cov}} 
\newcommand{\vech}{\mbox{vech}}
\newcommand{\pl}{\widetilde\ell}
\newcommand{\plkij}{\widetilde\ell_{k,k,\{i,j\}}}
\newcommand{\plklij}{\widetilde\ell_{k,l,\{i,j\}}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\Aavg}{A_{\textup{avg}}}
\newcommand{\Amax}{A_{\max}}
\newcommand{\avg}{\textup{avg}}


% Text in math
\newcommand{\rint}{\mathop{\mbox{rint}}}
\newcommand{\mdim}{\mbox{dim}}
\newcommand{\interior}{\textnormal{int}}
\newcommand{\cert}{\textnormal{cert}}
\newcommand{\su}{\sup\limits}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\tv}{{\tiny\mbox{TV}}}
\newcommand{\lip}{{\tiny\mbox{Lip}}}
\newcommand{\rank}{\textnormal{rank}}
\newcommand{\dimd}{m}
\newcommand{\defined}{\overset{\scalebox{0.75}{def}}{=}}


% \mathscr
\newcommand{\mA}{\mathscr{A}}
\newcommand{\mB}{\mathscr{B}}
\newcommand{\mC}{\mathscr{C}}
\newcommand{\mD}{\mathscr{D}}
\newcommand{\mE}{\mathscr{E}}
\newcommand{\mF}{\mathscr{F}}
\newcommand{\mG}{\mathscr{G}}
\newcommand{\mmG}{\mathfrak{N}}
\newcommand{\mH}{\mathscr{H}}
\newcommand{\mJ}{\mathscr{J}}
\newcommand{\mK}{\mathscr{K}}
\newcommand{\mL}{\mathscr{L}}
\newcommand{\mM}{\mathscr{M}}
\newcommand{\mN}{\mathscr{N}}
\newcommand{\mO}{\mathscr{O}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mQ}{\mathscr{Q}}
\newcommand{\mR}{\mathds{R}}
\newcommand{\mS}{\mathscr{S}}
\newcommand{\mT}{\mathscr{T}}
\newcommand{\mU}{\mathscr{U}}
\newcommand{\mV}{\mathscr{V}}
\newcommand{\mW}{\mathscr{W}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathscr{Y}}
\newcommand{\mZ}{\mathscr{Z}}


% \mathcal
\newcommand{\mcA}{\mathcal{A}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcD}{\mathcal{D}}
\newcommand{\mcE}{\mathcal{E}}
\newcommand{\mcF}{\mathcal{F}}
\newcommand{\mcG}{\mathcal{G}}
\newcommand{\mcH}{\mathcal{H}}
\newcommand{\mcI}{I}
%\newcommand{\mcI}{\mathcal{I}}
\newcommand{\mcJ}{\mathcal{J}}
\newcommand{\mcK}{\mathcal{K}}
\newcommand{\mcL}{\mathcal{L}}
\newcommand{\mcM}{\mathcal{M}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcP}{\mathcal{P}}
\newcommand{\mcQ}{\mathcal{Q}}
\newcommand{\mcR}{\mathcal{R}}
\newcommand{\mcS}{\mathds{S}}
\newcommand{\mcT}{\mathcal{T}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcV}{\mathcal{V}}
\newcommand{\mcW}{\mathcal{W}}
\newcommand{\mcX}{\mathcal{X}}
\newcommand{\mcY}{\mathcal{Y}}
\newcommand{\mcZ}{\mathcal{Z}}




%  \mathds
\newcommand{\mbA}{\mathds{A}}
\newcommand{\mbB}{\mathds{B}}
\newcommand{\mbC}{\mathds{C}}
\newcommand{\mbD}{\mathds{D}}
\newcommand{\mbE}{\mathds{E}}
\newcommand{\mbF}{\mathds{F}}
\newcommand{\mbG}{\mathds{G}}
\newcommand{\mbH}{\mathds{H}}
\newcommand{\mbI}{\mathds{I}}
\newcommand{\mbJ}{\mathds{J}}
\newcommand{\mbK}{\mathds{K}}
\newcommand{\mbL}{\mathds{L}}
\newcommand{\mbM}{\mathds{M}}
\newcommand{\mbN}{\mathds{N}}
\newcommand{\mbO}{\mathds{O}}
\newcommand{\mbP}{\mathds{P}}
\newcommand{\mbQ}{\mathds{Q}}
\newcommand{\mbR}{\mathds{R}}
\newcommand{\mbS}{\mathds{S}}
\newcommand{\mbT}{\mathds{T}}
\newcommand{\mbU}{\mathds{U}}
\newcommand{\mbV}{\mathds{V}}
\newcommand{\mbW}{\mathds{W}}
\newcommand{\mbX}{\mathds{X}}
\newcommand{\mbY}{\mathds{Y}}
\newcommand{\mbZ}{\mathds{Z}}


% \bm -- lowercase
\newcommand{\bma}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bmi}{\bm{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\mathscr{P}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}

% \bm -- uppercase 
\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}

% bold greek
\newcommand{\balpha}{\bm\alpha}
\newcommand{\bphi}{\mbox{\boldmath$\phi$}}
\newcommand{\bbeta}{\mbox{\boldmath$\beta$}}
\newcommand{\bgamma}{\mbox{\boldmath$\gamma$}}
\newcommand{\blambda}{\mbox{\boldmath$\lambda$}}
\newcommand{\brho}{\mbox{\boldmath$\rho$}}
\newcommand{\bmu}{\mbox{\boldmath$\mu$}}
\newcommand{\bomega}{\mbox{\boldmath$\omega$}}
\newcommand{\bsigma}{\mbox{\boldmath$\sigma$}}
\newcommand{\bSigma}{\mbox{\boldmath$\Sigma$}}
\newcommand{\bTheta}{\bm\Theta}
\newcommand{\bta}{\boldsymbol{\eta}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\hatbtheta}{\boldsymbol{\hat{\theta}}}
\newcommand{\bvartheta}{\mbox{\boldmath$\vartheta$}}
\newcommand{\bpi}{\mbox{\boldmath$\pi$}}
\newcommand{\bxi}{\mbox{\boldmath$\xi$}}
\newcommand{\bXi}{\mbox{\boldmath$\Xi$}}
\newcommand{\bPsi}{\mbox{\boldmath$\Psi$}}
\newcommand{\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand{\bLambda}{\mbox{\boldmath$\Lambda$}}
\newcommand{\bPhi}{\mbox{\boldmath$\Phi$}}
\newcommand{\bnu}{\mbox{\boldmath$\vartheta$}}
\newcommand{\bupsilon}{\mbox{\boldmath$\upsilon$}}
\newcommand{\bUpsilon}{\mbox{\boldmath$\Upsilon$}}



% General Math Symbols 
\newcommand{\msim}{\mathop{\rm \sim}}
\newcommand{\one}{\mathbbm{1}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\newcommand\orth{\protect\mathpalette{\protect\independenT}{\perp}}
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\tends}{\longrightarrow}
\newcommand{\tend}{\rightarrow}
\newcommand{\define}{\mathop{=}\limits^{\mbox{\tiny def}}}
\newcommand{\law}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize d}}}
\newcommand{\as}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize a.s.}}}
\newcommand{\ind}{\msim\limits^{\mbox{\tiny ind}}}
\newcommand{\iid}{\msim\limits^{\mbox{\tiny iid}}}
\renewcommand{\bar}{\overline}
\newcommand{\dsum}{\displaystyle\sum\limits}
\newcommand{\dint}{\displaystyle\int\limits}
\newcommand{\dprod}{\displaystyle\prod\limits}
\newcommand{\var}{\mathds{V}}
\newcommand{\cov}{\mathds{C}}
\newcommand{\norm}[1]{|\!|#1|\!|} 
\newcommand{\mnorm}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\natspace}{\bm{\mathfrak{N}}}
\newcommand{\mmax}{{\tiny \mbox{max}}}
\newcommand{\gradW}{\gamma_{W}(\nat_W, \bx)}
\newcommand{\GradW}{\gamma_{W}(\nat_W, \bX)}
\newcommand{\gradB}{\gamma_{B}(\nat_B, \bx)}
\newcommand{\GradB}{\gamma_{B}(\nat_B, \bX)}
\newcommand{\gradLW}{\gamma_{k,k}(\nat_W, \bx_{\mA_k})}
\newcommand{\gradLB}{\gamma_{k,l}(\nat_B, \bx_{\mA_k,\mA_l})}
\newcommand{\GradLW}{\gamma_{k,k}(\nat_W, \bX_{\mA_k})}
\newcommand{\GradLB}{\gamma_{k,l}(\nat_B, \bX_{\mA_k,\mA_l})}
\newcommand{\Lam}{\xi_{\epsilon^\star} \; \mbE \, \norm{\bY}_1}
\newcommand{\LamPL}{\widetilde\xi_{\epsilon^\star} \; \mbE \, \norm{\bY}_1}
\newcommand{\gradPL}{\widetilde\gamma_{\nat}(\bx)}
\newcommand{\GradPL}{\widetilde\gamma_{\nat}(\bX)}
\newcommand{\phiN}{\phi_N(\truth)}
\newcommand{\mbXkij}{\mbX_{k,k,\{i,j\}}^{\bx}} 
\newcommand{\mbXklij}{\mbX_{k,l,\{i,j\}}^{\bx}}
\newcommand{\mbEkij}{\mbE_{\{i,j\},\btheta_W}^{\bx}}
\newcommand{\mbEklij}{\mbE_{\{i,j\}, \btheta_B}^{\bx}}
\newcommand{\mlewprob}{\ldots}
\newcommand{\mlebprob}{\ldots}
\newcommand{\tbR}{\widetilde\bR}
\newcommand{\tbD}{\widetilde\bD}
\newcommand{\natw}{\nat_W}
\newcommand{\natb}{\nat_B}
\newcommand{\maxw}{\widetilde{\lambda}^{\star}_{\max,W}}
\newcommand{\minw}{\widetilde{\lambda}^{\epsilon}_{\min,W}}
\newcommand{\maxb}{\widetilde{\lambda}^{\star}_{\max,B}}
\newcommand{\minb}{\widetilde{\lambda}^{\epsilon}_{\min,B}}
\newcommand{\maxwe}{\widetilde{\lambda}^{\epsilon}_{\max,W}}
\newcommand{\maxbe}{\widetilde{\lambda}^{\epsilon}_{\max,B}}
\newcommand{\minwt}{\widetilde{\lambda}^{\star}_{\min,W}}
\newcommand{\minbt}{\widetilde{\lambda}^{\star}_{\min,B}}

\newtheorem{remark}{Remark}


% begin/end enviornment commands
\newcommand{\be}{\begin{equation}\arraycolsep=4pt\begin{array}{lllllllllllllllll}}
\newcommand{\beno}{\begin{equation}\arraycolsep=4pt\begin{array}{lllllllllllll}\nonumber}
\newcommand{\ee}{\end{array}\end{equation}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}


% Proof language / math env symbol commands -- to be used in \be \ee enviornments 
\renewcommand{\=}{&=&}





% Latex editor helpers
\newcommand{\dis}{\displaystyle}
\newcommand{\hide}[1]{}
\newcommand{\ghost}[1]{}
\newcommand{\alert}{\textcolor{red}}
\newcommand{\s}{\vspace{0.25cm}}
\newcommand{\hs}{\hspace{0.25cm}}
\newcommand{\lef}{\left(}
\newcommand{\rig}{\right)}
\newcommand{\cont}{\alert{Please continue here...}}
\newcommand{\fs}{\footnotesize}
\newcommand{\ti}{\tiny}



\newcounter{com}
\newenvironment{com}[1][]{\refstepcounter{com}\par\medskip\indent%
\textit{Remark~\thecom #1}. \rmfamily}{\medskip}

\newcounter{assumption}
\newenvironment{assumption}[1][]{\refstepcounter{assumption}\par\noindent%
\textbf{Assumption~\theassumption #1}. \rmfamily}{\medskip}


\newcommand{\nat}{\btheta}
\newcommand{\Nat}{\bTheta}




\newcounter{ttproof}
\setcounter{ttproof}{0}
\newcommand{\ttproof}{%
\addtocounter{ttproof}{1}%
{\medskip}\textsc{Proof of Theorem}{}
}

\newcounter{llproof}
\setcounter{llproof}{0}
\newcommand{\llproof}{%
\addtocounter{llproof}{1}%
{}\textsc{Proof of Lemma}{}
}



